Snowmass2021 Cosmic Frontier White Paper: Cosmological Simulations for Dark Matter Physics

Over the past several decades, unexpected astronomical discoveries have been fueling a new wave of particle model building and are inspiring the next generation of ever-more-sophisticated simulations to reveal the nature of Dark Matter (DM). This coincides with the advent of new observing facilities coming online, including JWST, the Rubin Observatory, the Nancy Grace Roman Space Telescope, and CMB-S4. The time is now to build a novel simulation program to interpret observations so that we can identify novel signatures of DM microphysics across a large dynamic range of length scales and cosmic time. This white paper identifies the key elements that are needed for such a simulation program. We identify areas of growth on both the particle theory side as well as the simulation algorithm and implementation side, so that we can robustly simulate the cosmic evolution of DM for well-motivated models. We recommend that simulations include a fully calibrated and well-tested treatment of baryonic physics, and that outputs should connect with observations in the space of observables. We identify the tools and methods currently available to make predictions and the path forward for building more of these tools. A strong cosmic DM simulation program is key to translating cosmological observations to robust constraints on DM fundamental physics, and provides a connection to lab-based probes of DM physics.

==> intro_old.tex <==
Astronomical observations over a wide variety of redshifts and size-scales attest to the existence of dark matter (DM) Evidence for dark matter has been made robust through multiple, orthogonal astrophysical observational probes (e.g., galaxy rotation curves, the Cosmic Microwave Background, gravitational lensing).  Dark matter is strong proof of physics beyond the standard model.  Given the lack of direct detection of dark matter in laboratory experiments, the both the astronomical community and the particle physics community has recently focused on constraining the fundamental characteristics of dark matter to narrow the possible parameter space of particle dark matter models. But the fundamental nature of DM remains unknown, and its existence implies new physics whose investigation centrally drives research at the intersection of astrophysics, cosmology, and particle physics. 

There have been major efforts in DM model-building to move beyond the standard weakly-interacting massive particle paradigm.

Many models are not only inspired by observations, but also predict striking signatures that can be uniquely tested with upcoming observational facilities.
Over the coming years, observations that probe the distribution of matter on various scales and the thermal history of the universe will reach improved sensitivity to DM interactions with the Standard Model, such as the DM annihilation and scattering cross sections as a function of DM mass, complementing the more traditional indirect and direct detection searches.
These observations are also crucial for understanding the properties of DM or a dark sector that only communicates with the visible sector through gravitational effects; for instance, they will target the free-streaming length of warm DM, the de-Broglie wavelength of fuzzy DM, DM interactions with a dark thermal bath, and DM self-interactions.

In the past decade, simulators have demonstrated that a realistic treatment of baryonic physics can solve many of the small scale problems of CDM.  Despite the successes, new challenges are emerging: 

Upcoming large-scale surveys---including galaxy surveys, measurements of the cosmic microwave background (CMB) temperature, polarization, and lensing, and line-intensity mapping---will shortly begin to reach sufficient raw sensitivity to potentially uncover DM signals that are invisible to present-day searches. Notably, the Legacy Survey of Space and Time (LSST) by the Vera C. Rubin Observatory, planned to begin in 2023, is designed to sensitively probe structure on a range of physical scales and stress-test a variety of beyond-CDM paradigms mentioned above.
Simons Observatory (SO), the next-generation ground-based CMB experiment is planned to begin the following year. It aims to dramatically improve constraints on physics beyond $\Lambda$CDM, including the presence of new light particle species, neutrino mass, and the overall thermal history of the universe, opening complementary early-universe windows into the physics of DM. 
In combination, these facilities will enable a suite of observational tests, providing constraints on various fundamental particle properties of DM and propelling future model-building efforts within the particle physics community.

However, further progress with observational searches for the fundamental nature of DM hinges on development of theory, simulation, and analysis tools to reliably identify beyond-CDM signals across physical scales and throughout cosmic history.  In this white paper we identify key needs for the upcoming decade:


%\vspace{-0.2cm}
\begin{itemize}

\item Collaboration between cosmological simulators and particle theorists
\item Algorithm development and code comparison tests
\item Simulations with full hydrodynamics for observational targets
\item Comparison of observations and simulations {\bf in the space of observables.}
\item Fast realization of observed systems for DM parameter constraints
\item Guidance to observers for promising signatures of DM physics.
\end{itemize}

